Experience Report: Deep Learning-based System Log Analysis for Anomaly Detection

Logs have been an imperative resource to ensure the reliability and continuity of many software systems, especially large-scale distributed systems. They faithfully record runtime information to facilitate system troubleshooting and behavior understanding. Due to the large scale and complexity of modern software systems, the volume of logs has reached an unprecedented level. Consequently, for log-based anomaly detection, conventional manual inspection methods or even traditional machine learning-based methods become impractical, which serve as a catalyst for the rapid development of deep learning-based solutions. However, there is currently a lack of rigorous comparison among the representative log-based anomaly detectors that resort to neural networks. Moreover, the re-implementation process demands non-trivial efforts, and bias can be easily introduced. To better understand the characteristics of different anomaly detectors, in this paper, we provide a comprehensive review and evaluation of five popular neural networks used by six state-of-the-art methods. Particularly, four of the selected methods are unsupervised, and the remaining two are supervised. These methods are evaluated with two publicly available log datasets, which contain nearly 16 million log messages and 0.4 million anomaly instances in total. We believe our work can serve as a basis in this field and contribute to future academic research and industrial applications.

==> bibliography_bak.tex <==
@inproceedings{chen2020towards,
  title={Towards intelligent incident management: why we need it and how we make it},
  author={Chen, Zhuangbin and Kang, Yu and Li, Liqun and Zhang, Xu and Zhang, Hongyu and Xu, Hui and Zhou, Yangfan and Yang, Li and others},
  booktitle={Proc. of ESEC/FSE'20},
  pages={1487--1497},
  year={2020}
}

@article{chenaiops,
  title={AIOps Innovations of Incident Management for Cloud Services},
  author={Chen, Zhuangbin and Kang, Yu and Gao, Feng and Yang, Li and Sun, Jeffrey and Xu, Zhangwei and Zhao, Pu and Qiao, Bo and Li, Liqun and Zhang, Xu and others},
  year={2020}
}

@inproceedings{zhang2019robust,
  title={Robust log-based anomaly detection on unstable log data},
  author={Zhang, Xu and Xu, Yong and Lin, Qingwei and Qiao, Bo and Zhang, Hongyu and Dang, Yingnong and Xie, Chunyu and Yang, Xinsheng and Cheng, Qian and Li, Ze and others},
  booktitle={Proc. of ESEC/FSE'19},
  pages={807--817},
  year={2019}
}

@inproceedings{lu2018detecting,
  title={Detecting anomaly in big data system logs using convolutional neural network},
  author={Lu, Siyang and Wei, Xiang and Li, Yandong and Wang, Liqiang},
  booktitle={Proc. of DASC/PiCom/DataCom/CyberSciTech'18},
  pages={151--158},
  year={2018},
  organization={IEEE}
}

@inproceedings{du2017deeplog,
  title={Deeplog: Anomaly detection and diagnosis from system logs through deep learning},
  author={Du, Min and Li, Feifei and Zheng, Guineng and Srikumar, Vivek},
  booktitle={Proc. of CCS'17},
  pages={1285--1298},
  year={2017}
}

@inproceedings{meng2019loganomaly,
  title={LogAnomaly: Unsupervised Detection of Sequential and Quantitative Anomalies in Unstructured Logs.},
  author={Meng, Weibin and Liu, Ying and Zhu, Yichen and Zhang, Shenglin and Pei, Dan and Liu, Yuqing and Chen, Yihao and Zhang, Ruizhi and Tao, Shimin and Sun, Pei and others},
  booktitle={Proc. of IJCAI'19},
  pages={4739--4745},
  year={2019}
}

@article{schuster1997bidirectional,
  title={Bidirectional recurrent neural networks},
  author={Schuster, Mike and Paliwal, Kuldip K},
  journal={IEEE transactions on Signal Processing},
  volume={45},
  number={11},
  pages={2673--2681},
  year={1997},
  publisher={Ieee}
}

@article{bahdanau2014neural,
  title={Neural machine translation by jointly learning to align and translate},
  author={Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1409.0473},
  year={2014}
}

@inproceedings{xu2009detecting,
  title={Detecting large-scale system problems by mining console logs},
  author={Xu, Wei and Huang, Ling and Fox, Armando and Patterson, David and Jordan, Michael I},
  booktitle={Proc. of SOSP'09},
  pages={117--132},
  year={2009}
}

@inproceedings{lin2016log,
  title={Log clustering based problem identification for online service systems},
  author={Lin, Qingwei and Zhang, Hongyu and Lou, Jian-Guang and Zhang, Yu and Chen, Xuewei},
  booktitle={Proc. of ICSE-C'16},
  pages={102--111},
  year={2016},
  organization={IEEE}
}

@inproceedings{lou2010mining,
  title={Mining Invariants from Console Logs for System Problem Detection.},
  author={Lou, Jian-Guang and Fu, Qiang and Yang, Shengqi and Xu, Ye and Li, Jiang},
  booktitle={Proc. of USENIXATC'10},
  pages={1--14},
  year={2010}
}

@inproceedings{he2016experience,
  title={Experience report: System log analysis for anomaly detection},
  author={He, Shilin and Zhu, Jieming and He, Pinjia and Lyu, Michael R},
  booktitle={Proc. of ISSRE'16},
  pages={207--218},
  year={2016},
  organization={IEEE}
}

@inproceedings{dang2019aiops,
  title={AIOps: real-world challenges and research innovations},
  author={Dang, Yingnong and Lin, Qingwei and Huang, Peng},
  booktitle={Proc. of ICSE-C'19},
  pages={4--5},
  year={2019},
  organization={IEEE}
}

@article{farzad2020unsupervised,
  title={Unsupervised log message anomaly detection},
  author={Farzad, Amir and Gulliver, T Aaron},
  journal={ICT Express},
  volume={6},
  number={3},
  pages={229--237},
  year={2020},
  publisher={Elsevier}
}

@article{nguyen2016integrating,
  title={Integrating distributional lexical contrast into word embeddings for antonym-synonym distinction},
  author={Nguyen, Kim Anh and Walde, Sabine Schulte im and Vu, Ngoc Thang},
  journal={arXiv preprint arXiv:1605.07766},
  year={2016}
}

@article{nedelkoski2020self,
  title={Self-attentive classification-based anomaly detection in unstructured logs},
  author={Nedelkoski, Sasho and Bogatinovski, Jasmin and Acker, Alexander and Cardoso, Jorge and Kao, Odej},
  journal={arXiv preprint arXiv:2008.09340},
  year={2020}
}

@article{hashemi2021detecting,
  title={Detecting Anomalies in Software Execution Logs with Siamese Network},
  author={Hashemi, Shayan and M{\"a}ntyl{\"a}, Mika},
  journal={arXiv preprint arXiv:2102.01452},
  year={2021}
}

@inproceedings{zhou2019latent,
  title={Latent error prediction and fault localization for microservice applications by learning from system trace logs},
  author={Zhou, Xiang and Peng, Xin and Xie, Tao and Sun, Jun and Ji, Chao and Liu, Dewei and Xiang, Qilin and He, Chuan},
  booktitle={Proc. of ESEC/FSE'19},
  pages={683--694},
  year={2019}
}

@inproceedings{prewett2003analyzing,
  title={Analyzing cluster log files using logsurfer},
  author={Prewett, James E},
  booktitle={Proc. of the 4th Annual Conference on Linux Clusters},
  year={2003},
  organization={Citeseer}
}

@inproceedings{rouillard2004real,
  title={Real-time Log File Analysis Using the Simple Event Correlator (SEC).},
  author={Rouillard, John P},
  booktitle={Proc. of LISA'04},
  volume={4},
  pages={133--150},
  year={2004}
}

@inproceedings{hansen1993automated,
  title={Automated System Monitoring and Notification with Swatch.},
  author={Hansen, Stephen E and Atkins, E Todd},
  booktitle={Proc. of LISA'93},
  volume={93},
  pages={145--152},
  year={1993}
}

@inproceedings{liang2007failure,
  title={Failure prediction in ibm bluegene/l event logs},
  author={Liang, Yinglung and Zhang, Yanyong and Xiong, Hui and Sahoo, Ramendra},
  booktitle={Proc. of ICDM'07},
  pages={583--588},
  year={2007},
  organization={IEEE}
}

@inproceedings{zhu2019tools,
  title={Tools and benchmarks for automated log parsing},
  author={Zhu, Jieming and He, Shilin and Liu, Jinyang and He, Pinjia and Xie, Qi and Zheng, Zibin and Lyu, Michael R},
  booktitle={Proc. of ICSE-SEIP'19},
  pages={121--130},
  year={2019},
  organization={IEEE}
}

@inproceedings{nagappan2010abstracting,
  title={Abstracting log lines to log event types for mining software system logs},
  author={Nagappan, Meiyappan and Vouk, Mladen A},
  booktitle={Proc. of MSR'10},
  pages={114--117},
  year={2010},
  organization={IEEE}
}

@inproceedings{vaarandi2003data,
  title={A data clustering algorithm for mining patterns from event logs},
  author={Vaarandi, Risto},
  booktitle={Proc. of IPOM'03},
  pages={119--126},
  year={2003},
  organization={Ieee}
}

@inproceedings{fu2009execution,
  title={Execution anomaly detection in distributed systems through unstructured log analysis},
  author={Fu, Qiang and Lou, Jian-Guang and Wang, Yi and Li, Jiang},
  booktitle={Proc. of ICDM'09},
  pages={149--158},
  year={2009},
  organization={IEEE}
}

@inproceedings{vaarandi2015logcluster,
  title={Logcluster-a data clustering and pattern mining algorithm for event logs},
  author={Vaarandi, Risto and Pihelgas, Mauno},
  booktitle={Proc. of CNSM'15},
  pages={1--7},
  year={2015},
  organization={IEEE}
}

@article{dai2020logram,
  title={Logram: Efficient log parsing using n-gram dictionaries},
  author={Dai, Hetong and Li, Heng and Chen, Che Shao and Shang, Weiyi and Chen, Tse-Hsun},
  journal={TSE},
  year={2020},
  publisher={IEEE}
}

@inproceedings{jiang2008abstracting,
  title={Abstracting execution logs to execution events for enterprise applications (short paper)},
  author={Jiang, Zhen Ming and Hassan, Ahmed E and Flora, Parminder and Hamann, Gilbert},
  booktitle={Proc. of QSIC'08},
  pages={181--186},
  year={2008},
  organization={IEEE}
}

@inproceedings{he2017drain,
  title={Drain: An online log parsing approach with fixed depth tree},
  author={He, Pinjia and Zhu, Jieming and Zheng, Zibin and Lyu, Michael R},
  booktitle={Proc. of ICWS'17},
  pages={33--40},
  year={2017},
  organization={IEEE}
}

@article{joulin2016fasttext,
  title={Fasttext. zip: Compressing text classification models},
  author={Joulin, Armand and Grave, Edouard and Bojanowski, Piotr and Douze, Matthijs and J{\'e}gou, H{\'e}rve and Mikolov, Tomas},
  journal={arXiv preprint arXiv:1612.03651},
  year={2016}
}

@inproceedings{pennington2014glove,
  title={Glove: Global vectors for word representation},
  author={Pennington, Jeffrey and Socher, Richard and Manning, Christopher D},
  booktitle={Proc. of EMNLP'14},
  pages={1532--1543},
  year={2014}
}

@inproceedings{liu2008isolation,
  title={Isolation forest},
  author={Liu, Fei Tony and Ting, Kai Ming and Zhou, Zhi-Hua},
  booktitle={Proc. of ICDM'08},
  pages={413--422},
  year={2008},
  organization={IEEE}
}

@techreport{rumelhart1985learning,
  title={Learning internal representations by error propagation},
  author={Rumelhart, David E and Hinton, Geoffrey E and Williams, Ronald J},
  year={1985},
  institution={California Univ San Diego La Jolla Inst for Cognitive Science}
}

@inproceedings{NIPS2017_3f5ee243,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Proc. of NIPS'17},
 title = {Attention is All you Need},
 year = {2017}
}

@misc{pytorch,
  author = {PyTorch},
  year   = {2016},
  url    = {https://pytorch.org/},
  lastaccessed ={May, 2021}
}

@misc{tensorflow,
  author = {Tensorflow},
  year   = {2015},
  url    = {https://www.tensorflow.org/},
  lastaccessed ={May, 2021}
}

@article{he2020loghub,
  title={Loghub: a large collection of system log datasets towards automated log analytics},
  author={He, Shilin and Zhu, Jieming and He, Pinjia and Lyu, Michael R},
  journal={arXiv preprint arXiv:2008.06448},
  year={2020}
}

@inproceedings{oliner2007supercomputers,
  title={What supercomputers say: A study of five system logs},
  author={Oliner, Adam and Stearley, Jon},
  booktitle={Proc. of DSN'07},
  pages={575--584},
  year={2007},
  organization={IEEE}
}

@inproceedings{yen2019causalconvlstm,
  title={CausalConvLSTM: Semi-supervised log anomaly detection through sequence modeling},
  author={Yen, Steven and Moh, Melody and Moh, Teng-Sheng},
  booktitle={Proc. of ICMLA'19},
  pages={1334--1341},
  year={2019},
  organization={IEEE}
}

@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proc. of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={Ieee}
}

@inproceedings{messaoudi2018search,
  title={A search-based approach for accurate identification of log message formats},
  author={Messaoudi, Salma and Panichella, Annibale and Bianculli, Domenico and Briand, Lionel and Sasnauskas, Raimondas},
  booktitle={Proc. of ICPC'18},
  pages={167--177},
  year={2018}
}

@inproceedings{du2016spell,
  title={Spell: Streaming parsing of system event logs},
  author={Du, Min and Li, Feifei},
  booktitle={Proc. of ICDM'16},
  pages={859--864},
  year={2016},
  organization={IEEE}
}

@inproceedings{mizutani2013incremental,
  title={Incremental mining of system log format},
  author={Mizutani, Masayoshi},
  booktitle={Proc. of SCC'13},
  pages={595--602},
  year={2013},
  organization={IEEE}
}

@inproceedings{he2018identifying,
  title={Identifying impactful service system problems via log analysis},
  author={He, Shilin and Lin, Qingwei and Lou, Jian-Guang and Zhang, Hongyu and Lyu, Michael R and Zhang, Dongmei},
  booktitle={Proc. of ESEC/FSE'18},
  pages={60--70},
  year={2018}
}

@article{xia2021loggan,
  title={LogGAN: A log-level generative adversarial network for anomaly detection using permutation event modeling},
  author={Xia, Bin and Bai, Yuxuan and Yin, Junjie and Li, Yun and Xu, Jian},
  journal={Information Systems Frontiers},
  volume={23},
  number={2},
  pages={285--298},
  year={2021},
  publisher={Springer}
}

@inproceedings{yang2021semi,
  title={Semi-supervised log-based anomaly detection via probabilistic label estimation},
  author={Yang, Lin and Chen, Junjie and Wang, Zan and Wang, Weijing and Jiang, Jiajun and Dong, Xuyuan and Zhang, Wenbin},
  booktitle={Proc. of ICSE'21},
  pages={1448--1460},
  year={2021},
  organization={IEEE}
}

@inproceedings{yuan2012conservative,
  title={Be conservative: Enhancing failure diagnosis with proactive logging},
  author={Yuan, Ding and Park, Soyeon and Huang, Peng and Liu, Yang and Lee, Michael M and Tang, Xiaoming and Zhou, Yuanyuan and Savage, Stefan},
  booktitle={Proc. of OSDI'12},
  pages={293--306},
  year={2012}
}

@inproceedings{fu2014developers,
  title={Where do developers log? an empirical study on logging practices in industry},
  author={Fu, Qiang and Zhu, Jieming and Hu, Wenlu and Lou, Jian-Guang and Ding, Rui and Lin, Qingwei and Zhang, Dongmei and Xie, Tao},
  booktitle={Proc. of ICSE-C'14},
  pages={24--33},
  year={2014}
}

@inproceedings{zhu2015learning,
  title={Learning to log: Helping developers make informed logging decisions},
  author={Zhu, Jieming and He, Pinjia and Fu, Qiang and Zhang, Hongyu and Lyu, Michael R and Zhang, Dongmei},
  booktitle={Proc. of ICSE'15},
  volume={1},
  pages={415--425},
  year={2015},
  organization={IEEE}
}

@inproceedings{yang2021interview,
  title={An interview study of how developers use execution logs in embedded software engineering},
  author={Yang, Nan and Schiffelers, Ramon and Lukkien, Johan},
  booktitle={Proc. of ICSE-SEIP'21},
  pages={61--70},
  year={2021},
  organization={IEEE}
}

@article{candido2019contemporary,
  title={Contemporary software monitoring: A systematic literature review},
  author={Candido, Jeanderson and Aniche, Maur{\'\i}cio and van Deursen, Arie},
  journal={arXiv e-prints},
  pages={arXiv--1912},
  year={2019}
}

@article{khan2016cloud,
  title={Cloud log forensics: foundations, state of the art, and future directions},
  author={Khan, Suleman and Gani, Abdullah and Wahab, Ainuddin Wahid Abdul and Bagiwa, Mustapha Aminu and Shiraz, Muhammad and Khan, Samee U and Buyya, Rajkumar and Zomaya, Albert Y},
  journal={CSUR},
  volume={49},
  number={1},
  pages={1--42},
  year={2016},
  publisher={ACM New York, NY, USA}
}

@article{zeng2016computer,
  title={Computer operating system logging and security issues: a survey},
  author={Zeng, Lei and Xiao, Yang and Chen, Hui and Sun, Bo and Han, Wenlin},
  journal={Security and communication networks},
  volume={9},
  number={17},
  pages={4804--4821},
  year={2016},
  publisher={Wiley Online Library}
}

@article{landauer2020system,
  title={System log clustering approaches for cyber security applications: A survey},
  author={Landauer, Max and Skopik, Florian and Wurzenberger, Markus and Rauber, Andreas},
  journal={Computers \& Security},
  volume={92},
  pages={101739},
  year={2020},
  publisher={Elsevier}
}

@article{russo2015mining,
  title={Mining system logs to learn error predictors: a case study of a telemetry system},
  author={Russo, Barbara and Succi, Giancarlo and Pedrycz, Witold},
  journal={Empirical Software Engineering},
  volume={20},
  number={4},
  pages={879--927},
  year={2015},
  publisher={Springer}
}

@inproceedings{sahoo2003critical,
  title={Critical event prediction for proactive management in large-scale computer clusters},
  author={Sahoo, Ramendra K and Oliner, Adam J and Rish, Irina and Gupta, Manish and Moreira, Jos{\'e} E and Ma, Sheng and Vilalta, Ricardo and Sivasubramaniam, Anand},
  booktitle={Proc. of SIGKDD'03},
  pages={426--435},
  year={2003}
}

@inproceedings{yuan2010sherlog,
  title={Sherlog: error diagnosis by connecting clues from run-time logs},
  author={Yuan, Ding and Mai, Haohui and Xiong, Weiwei and Tan, Lin and Zhou, Yuanyuan and Pasupathy, Shankar},
  booktitle={Proc. of ASPLOS'10},
  pages={143--154},
  year={2010}
}

@inproceedings{chen2018automated,
  title={An automated approach to estimating code coverage measures via execution logs},
  author={Chen, Boyuan and Song, Jian and Xu, Peng and Hu, Xing and Jiang, Zhen Ming},
  booktitle={Proc. of ASE'18},
  pages={305--316},
  year={2018}
}

@inproceedings{nandi2016anomaly,
  title={Anomaly detection using program control flow graph mining from execution logs},
  author={Nandi, Animesh and Mandal, Atri and Atreja, Shubham and Dasgupta, Gargi B and Bhattacharya, Subhrajit},
  booktitle={Proc. of SIGKDD'16},
  pages={215--224},
  year={2016}
}

@inproceedings{zhao2021empirical,
  title={An empirical investigation of practical log anomaly detection for online service systems},
  author={Zhao, Nengwen and Wang, Honglin and Li, Zeyan and Peng, Xiao and Wang, Gang and Pan, Zhu and others},
  booktitle={Proc. of ESEC/FSE'21},
  pages={1404--1415},
  year={2021}
}

@article{he2021survey,
  title={A survey on automated log analysis for reliability engineering},
  author={He, Shilin and He, Pinjia and Chen, Zhuangbin and Yang, Tianyi and Su, Yuxin and Lyu, Michael R},
  journal={CSUR},
  volume={54},
  number={6},
  pages={1--37},
  year={2021},
  publisher={ACM New York, NY, USA}
}

@inproceedings{liu2019logzip,
  title={Logzip: extracting hidden structures via iterative clustering for log compression},
  author={Liu, Jinyang and Zhu, Jieming and He, Shilin and He, Pinjia and Zheng, Zibin and Lyu, Michael R},
  booktitle={Proc. of ASE'19},
  pages={863--873},
  year={2019},
  organization={IEEE}
}

@misc{message_templates,
  author = {Message Templates Community},
  title  = {Message Templates},
  year   = {2011},
  url    = {https://messagetemplates.org/},
  lastaccessed ={October, 2021}
}

@misc{kafka,
  author = {Apache Software Foundation},
  title  = {Apache Kafka},
  year   = {2011},
  url    = {https://kafka.apache.org/},
  lastaccessed ={October, 2021}
}

@misc{flink,
  author = {Apache Flink},
  year   = {2011},
  url    = {https://flink.apache.org/},
  lastaccessed ={October, 2021}
}

@misc{hdfs,
  author = {HDFS},
  year   = {2006},
  url    = {https://hadoop.apache.org/docs/r1.2.1/hdfs_design.html},
  lastaccessed ={October, 2021}
}

@misc{prometheus,
  author = {Prometheus},
  year   = {2012},
  url    = {https://prometheus.io/},
  lastaccessed ={October, 2021}
}


==> secs/discussion.tex <==
\section{Discussion}

discuss data shuffle? call for more ways to learn unseen data. Current way of leveraging log semantics is not reasonable.


Pretrained word vectors do not bring noticeable performance gain. One reason is that many words cannot be found.
